Bio-JOIE: Joint Representation Learning of Biological Knowledge Bases

The widespread of Coronavirus has led to a worldwide pandemic with a high mortality rate. Currently, the knowledge accumulated from different studies about this virus is very limited. Leveraging a wide-range of biological knowledge, such as gene ontology and protein-protein interaction (PPI) networks from other closely related species presents a vital approach to infer the molecular impact of a new species. In this paper, we propose the transferred multi-relational embedding model Bio-JOIE to capture the knowledge of gene ontology and PPI networks, which demonstrates superb capability in modeling the SARS-CoV-2-human protein interactions. Bio-JOIE jointly trains two model components. The knowledge model encodes the relational facts from the protein and GO domains into separated embedding spaces, using a hierarchy-aware encoding technique employed for the GO terms. On top of that, the transfer model learns a non-linear transformation to transfer the knowledge of PPIs and gene ontology annotations across their embedding spaces. By leveraging only structured knowledge, Bio-JOIE significantly outperforms existing state-of-the-art methods in PPI type prediction on multiple species. Furthermore, we also demonstrate the potential of leveraging the learned representations on clustering proteins with enzymatic function into enzyme commission families. Finally, we show that Bio-JOIE can accurately identify PPIs between the SARS-CoV-2 proteins and human proteins, providing valuable insights for advancing research on this new disease.

==> sections/04_Discussion.tex <==
\section{Discussion}

\todo{We include the parameter study in discussion such as dimensionality, if possible and space allowed} 

\junheng{This section is not applied in the paper.}

\stitle{Dimensionality}

==> tables/covid-binary.tex <==
\begin{table}[htbp]
\centering
\caption{F-1 score on \covid-Human PPI interaction classification. \todo{Pending results updates.}}
\vspace{-6pt}
%\resizebox{\linewidth}{!}{
%\setlength\tabcolsep{3pt}{
\small
\begin{tabular}{c|c|c|c|c}
\newtoprule
{Input} &  S1 & S2 & S3 & S4 \\
\newtoprule
Non-GO    & 0.6737 & 0.7004 & 0.6918 & 0.6997 \\
\newmidrule
BP      & 0.6869    & 0.7286    & 0.7292    & 0.7130 \\
CC      & 0.6927    & 0.7577    & 0.7380    & 0.7025 \\
MF      & 0.6708    & 0.7099    & 0.7195    & 0.7038 \\
\newmidrule
BP+CC   & 0.7013	& 0.7283	& 0.6966	& 0.6679\\
BP+MF   & 0.6186	& 0.7148	& 0.6622	& 0.6442\\
\rowcolor{shadecolor} 
CC+MF   & 0.7425    & \textbf{0.7679}    & 0.7500    & 0.7555 \\
\newmidrule
All Go  & 0.7256    & 0.7339    & 0.6866	& 0.6573 \\
\newbottomrule
\end{tabular}
%}
\label{tab:covid-binary}
\end{table}

==> tables/ec_clusters.tex <==
\begin{table}[htbp]
\centering
\caption{Results of top-level EC clustering effects on learning yeast protein embeddings. \todo{Delete transductive./Add second-level EC.}}
%\resizebox{\linewidth}{!}{
%\setlength\tabcolsep{3pt}{
\small
\begin{tabular}{c|c|cc}
\newtoprule
\multirow{2}{*}{ \tabincell{c}{\textbf{Setting}}} & \multirow{2}{*}{ \tabincell{c}{\textbf{Model}}} & \multicolumn{2}{c}{ \textbf{Top-level EC}} \\
& & ARI & Purity  \\
\newmidrule
\multirow{6}{*}{ \tabincell{c}{Transductive}}
& Onto2Vec (Parent)    & 0.0170 & 0.3324 \\
& Onto2Vec (Ancestor)  & 0.0413	& 0.3627 \\
& Onto2Vec (Sum)  	 	& 0.0157 & 0.3015 \\
& Onto2Vec (Mean)   	& 0.0181 & 0.2848 \\
& \modelname (KM only)  & 0.0193 & 0.2780 \\
& \modelname			& \textbf{0.0988} & \textbf{0.3998} \\
\newmidrule
\multirow{6}{*}{ \tabincell{c}{Inductive}}  
& Onto2Vec (Parent)    & 0.0053	& 0.2452  \\
& Onto2Vec (Ancestor)  & 0.0366 & 0.3022  \\
& Onto2Vec (Sum)  	 	& 0.0170 & 0.3242 \\
& Onto2Vec (Mean)   	& 0.0147 & 0.2616 \\
& \modelname (KM only)  & 0.0204 & 0.2514 \\
& \modelname			& \textbf{0.0507} & \textbf{0.3306} \\
\newbottomrule
\end{tabular}
%}
\label{tab:ec_cluster}
\end{table}

==> tables/ppi_covid.tex <==
\begin{table}[htbp]
\centering
\caption{PPI type prediction accuracy evaluated on \covid-Human interactions. \todo{Results updates pending.}}
\vspace{-8pt}
\resizebox{\linewidth}{!}{
%\setlength\tabcolsep{3pt}{
\small
\begin{tabular}{c|c|c}
\newtoprule
\textbf{Setting} & \textbf{Model Input} & \textbf{Accuracy} \\
\newmidrule
\multirow{4}{*}{ \tabincell{c}{KM Only}}  & \covid-Human PPIs &  0.519\\
& \covid-Human PPIs with 1-hop protein PPIs & 0.649\\
& \covid-Human PPIs with  all other human PPIs & 0.657 \\
&  \covid-Human proteins with all-species PPIs & 0.605 \\
\newmidrule
\multirow{4}{*}{ \tabincell{c}{KM+TM}}  & \covid-Human PPIs &  0.670\\
& \covid-Human PPIs with 1-hop protein PPIs & 0.708 \\
& \covid-Human PPIs with  all other human PPIs & \textbf{0.720} \\
& \covid-Human proteins with all-species PPIs &  0.669\\
\newbottomrule
\end{tabular}
}
\label{tab:ppi-covid}
\end{table}
